Parallel Algebraic Effect Handlers

Algebraic effects and handlers support composable and structured control-flow abstraction. However, existing designs of algebraic effects often require effects to be executed sequentially. This paper studies parallel algebraic effect handlers. In particular, we formalize {\lambda}p, an untyped lambda calculus which models two key features, effect handlers and parallelizable computations, the latter of which takes the form of a for expression as inspired by the Dex programming language. We present various interesting examples expressible in our calculus, and provide a Haskell implementation. We hope this paper provides a basis for future designs and implementations of parallel algebraic effect handlers.

==> ott-rules.tex <==
% template
\newcommand{\ottdruletemplate}[1]{\ottdrule[#1]{%
\ottpremise{A}
}{%
B
}{%
{\ottdrulename{template}}{}%
}}

\newcommand{\typing}[4]{{#1} \vdash {#2} : {#3}~ |~ {#4}}
\newcommand{\vtyping}[3]{{#1} \vdash_{v} {#2} : {#3}}
\newcommand{\htyping}[5]{{#1} \vdash_{h} {#2} : {#3}{#4}{#5}}

\newcommand{\ottdruletXXvar}[1]{\ottdrule[#1]{%
\ottpremise{x:\tau \in \Gamma}
}{%
\vtyping{\Gamma}{x}{\tau} 
}{%
{\ottdrulename{t\_var}}{}%
}}

\newcommand{\ottdruletXXint}[1]{\ottdrule[#1]{%
\ottpremise{}
}{%
\vtyping{\Gamma}{n}{\integer} 
}{%
{\ottdrulename{t\_int}}{}%
}}

\newcommand{\ottdruletXXlam}[1]{\ottdrule[#1]{%
\ottpremise{\typing{\Gamma, x:\tau_1}{e}{\tau_2}{\epsilon}}
}{%
\vtyping{\Gamma}{\lambda x:\tau_1.~e}{\tau_1 \to \epsilon~ \tau_2} 
}{%
{\ottdrulename{t\_lam}}{}%
}}

\newcommand{\ottdruletXXapp}[1]{\ottdrule[#1]{%
\ottpremise{\typing{\Gamma}{e_1}{\tau_1 \to \epsilon~ \tau_2}{\epsilon}}
\ottpremise{\typing{\Gamma}{e_2}{\tau_1}{\epsilon}}
}{%
\typing{\Gamma}{e_1~e_2}{\tau_2}{\epsilon}
}{%
{\ottdrulename{t\_app}}{}%
}}

\newcommand{\ottdruletXXperform}[1]{\ottdrule[#1]{%
\ottpremise{\op : \tau_1 \to \tau_2 \in \Sigma(l)}
}{%
\vtyping{\Gamma}{\perform~\op }{\tau_1 \to \langle l | \epsilon \rangle \tau_2 }
}{%
{\ottdrulename{t\_perform}}{}%
}}


\newcommand{\ottdruletXXfor}[1]{\ottdrule[#1]{%
\ottpremise{\typing{\Gamma,x:\fin{n}}{e}{\tau}{\epsilon}}
}{%
\typing{\Gamma}{\for~x:\fin{n}.~e }{ \fin{n} \Rightarrow \tau_a }{\epsilon}
}{%
{\ottdrulename{t\_for}}{}%
}}

\newcommand{\ottdruletXXhandler}[1]{\ottdrule[#1]{%
\ottpremise{ \op: \tau_1 \to \tau_2 \in \Sigma(l) }
\ottpremise{ \vtyping{\Gamma}{f_1}{\tau \to \tau_r} }
\ottpremise{ \vtyping{\Gamma}{f_2}{\tau_1 \to \epsilon~ (\tau_2 \to \epsilon~ \tau_r) \to \epsilon~ \tau_r } }
\ottpremise{ \vtyping{\Gamma}{f_3}{ (\fin{n} \to \epsilon~ \tau_a) \to \epsilon~ ((\fin{n} \Rightarrow \tau_a) \to \epsilon~ \tau_r) \to \epsilon~ \tau_r } }
}{%
\vtyping{\Gamma}{\handler~\{ \return \mapsto f_1, \op \mapsto f_2, \traverse \mapsto f_3\} }{ (() \to \effect{l|\epsilon} \tau) \to \epsilon~\tau_r }
}{%
{\ottdrulename{t\_handler}}{}%
}}

